Unifying Ensemble Methods for Q-learning via Social Choice Theory

Ensemble methods have been widely applied in Reinforcement Learning (RL) in order to enhance stability, increase convergence speed, and improve exploration. These methods typically work by employing an aggregation mechanism over actions of different RL algorithms. We show that a variety of these methods can be unified by drawing parallels from committee voting rules in Social Choice Theory. We map the problem of designing an action aggregation mechanism in an ensemble method to a voting problem which, under different voting rules, yield popular ensemble-based RL algorithms like Majority Voting Q-learning or Bootstrapped Q-learning. Our unification framework, in turn, allows us to design new ensemble-RL algorithms with better performance. For instance, we map two diversity-centered committee voting rules, namely Single Non-Transferable Voting Rule and Chamberlin-Courant Rule, into new RL algorithms that demonstrate excellent exploratory behavior in our experiments.

==> acknowledgement.tex <==
% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

%TODO: Add this section


==> deepexperiments.tex <==
\section{Experiments}

%TODO: Add this section

==> related.tex <==
% !TEX root = osrl.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}

\cite{Wiering:2008} 

==> results.tex <==
\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/ijcai2019/images/mdp-v5-Bloc-SNTV.png}
        \subcaption{\label{fig:comparision-Bloc-SNTV} Running average of rewards vs time-steps for Bloc, SNTV and Majority Voting Q-learning.}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/ijcai2019/images/mdp-v5-Broda-CCR.png}
        \subcaption{\label{fig:comparision-Broda-CCR} Running average of rewards vs time-steps for Broda, CCR and Rank Voting Q-learning}
    \end{subfigure}
    \caption{\label{fig:comparision} Comparison of ensemble Q-learning algorithms for increasing action-set sizes.}
\end{figure*}

\begin{table*}[hbt!]
    \centering
    \begin{tabular}{lcccccccc}
        \hline 
                                      & \multicolumn{4}{c}{single-winner voting}  & \multicolumn{4}{c}{multi-winner voting}      \\
        \cmidrule(l){2-5} \cmidrule(l){6-9} 
                                      & Average & Rank & Majority & Lottery        & Bloc & Broda & SNTV          & CCR           \\ 
        \hline
        MiniGrid-DoorKey-16x16-v0      & 0.08    & 0.06 & 0.37     & 0.38           & 0.41 & 0.11  & 0.49          & \textbf{0.58} \\
        MiniGrid-MultiRoom-N6-v0       & 0.00    & 0.01 & 0.13     & \textbf{0.47}  & 0.40 & 0.00  & \textbf{0.47} & \textbf{0.47} \\
        MiniGrid-KeyCorridorS4R3-v0    & 0.10    & 0.09 & 0.53     & 0.90           & 0.22 & 0.13  & \textbf{0.92} & \textbf{0.92} \\
        MiniGrid-ObstructedMaze-2Dl-v0 & 0.07    & 0.08 & 0.20     & 0.52           & 0.16 & 0.06  & 0.63          & \textbf{0.64} \\
        \hline
    \end{tabular}
    \caption{\label{tab:result-comparision}Maximum exponential moving average across 48 seeds.}
\end{table*}
